MMAU: A Holistic Benchmark of Agent Capabilities Across Diverse Domains

Recent advances in large language models (LLMs) have increased the demand for comprehensive benchmarks to evaluate their capabilities as human-like agents. Existing benchmarks, while useful, often focus on specific application scenarios, emphasizing task completion but failing to dissect the underlying skills that drive these outcomes. This lack of granularity makes it difficult to deeply discern where failures stem from. Additionally, setting up these environments requires considerable effort, and issues of unreliability and reproducibility sometimes arise, especially in interactive tasks. To address these limitations, we introduce the Massive Multitask Agent Understanding (MMAU) benchmark, featuring comprehensive offline tasks that eliminate the need for complex environment setups. It evaluates models across five domains, including Tool-use, Directed Acyclic Graph (DAG) QA, Data Science and Machine Learning coding, Contest-level programming and Mathematics, and covers five essential capabilities: Understanding, Reasoning, Planning, Problem-solving, and Self-correction. With a total of 20 meticulously designed tasks encompassing over 3K distinct prompts, MMAU provides a comprehensive framework for evaluating the strengths and limitations of LLM agents. By testing 18 representative models on MMAU, we provide deep and insightful analyses. Ultimately, MMAU not only sheds light on the capabilities and limitations of LLM agents but also enhances the interpretability of their performance. Datasets and evaluation scripts of MMAU are released at https://github.com/apple/axlearn/tree/main/docs/research/mmau.

==> sections/tool_use/exp_setup.tex <==
\textbf{Experiment Setup for Tool Use}

% Our in-house tool use dataset consists of 407 single-step and 256 multi-step tool use conversations. Out of the 407 single-step tool use conversations, 224 require making parallel tool calls. We adapt these examples to test the following capabilities.

% \textit{Function calling execution}
% The standard function calling protocol involves the following steps.
% \begin{itemize}
%     \item The user sends a query to the agent model along with a list of potential functions including description of their purposes and parameters.
%     \item The agent then responds with either natural language or appropriate use of functions.
%     \item In case of function call, the functions are invoked according to the agent either by the user or by the agent directly, and the result is submitted back to the agent model.
%     \item The agent can then conclude with the given information or continue the conversation with follow up questions or additional function calls.
% \end{itemize}
 
% Benchmarking agent tool use following the above protocol requires an interactive environment where the functions can be reliably executed and the agent's follow up questions can be answered. To simplify the evaluation process, we instead  evaluate the model's response at each assistant turn (i.e., where a function call is expected), conditioning on the ground-truth versions of all previous user or assistant turns. 
% For evaluation, we check if the model's tool call matches that of the ground truth.
% A match is defined as 
% 1. calling the same function, and 2. calling with the same parameters.
% To compare the predicted and the ground truth parameter values, we perform string normalization including stripping punctuation, white spaces and converting to lower case.
% In some cases where the parameter value can have open-ended, semantically equivalent forms, we define example-specific match rules to accommodate valid alternatives.

\textit{Function calling plan}

\textit{Self-correction}

